Design of a Lambda configuration in artificial coherent nanostructures

The implementation of a three-level Lambda System in artificial atoms would allow to perform advanced control tasks typical of quantum optics in the solid state realm, with photons in the $\mathrm{\mu m}$/mm range. However hardware constraints put an obstacle since protection from decoherence is often conflicting with efficient coupling to external fields. We address the problem of performing conventional STImulated Raman Adiabatic Passage (STIRAP) in the presence of low-frequency noise. We propose two strategies to defeat decoherence, based on "optimal symmetry breaking" and dynamical decoupling. We suggest how to apply to the different implementations of superconducting artificial atoms, stressing the key role of non-Markovianity.

==> rjp_mathdefs.tex <==
%This file contains a hopefully ever growing collection of command shortcuts and even new LaTeX commands (especially for math mode),
%that are currently in use and accepted by Romanian Journal of Physics.
% Last modified: 08/09/2013 (dd/mm/yyyy)
%
% Environment and general command shortcuts
\providecommand{\beq}[1][\@empty]{\def\@ttoken{#1}\begin{equation}\dbg@ut{\@ttoken}\ifx\@empty#1 \else\label{#1}\fi}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}
%
% Various other operators
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Img}{Im}
\DeclareMathOperator{\Rel}{Re}
\DeclareMathOperator{\ee}{e}
%
% Elliptic Jacobi functions - obsolete, do not use! (see below)
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}
%
% Mathematical operators and various symbols
\DeclareMathOperator{\ddiv}{div}
\DeclareMathOperator{\grad}{grad}
% Replaceable by \tanh^{-1}
% Hyperbolic functions
\DeclareMathOperator{\artanh}{artanh}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\cosech}{csch}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\cosec}{cosec}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}
% Partial derivative
\providecommand{\pd}{\ensuremath{\partial}}
% To be eliminated in future versions!
\providecommand{\dd}{\ensuremath{\mathrm{d}}}
\providecommand{\id}{\ensuremath{\;\mathrm{d}}}
% Full derivative
\providecommand{\fd}{\ensuremath{\mathrm{d}}}
% Bras and Kets
\providecommand{\bra}[1]{\ensuremath{\left<#1\right|}}
\providecommand{\ket}[1]{\ensuremath{\left|#1\right>}}
% the \braket command is thought to be the matrix element of operator #1 for state #2 (left) and state #3 (right)
\providecommand{\braket}[3]{\ensuremath{\left<#2|#1|#3\right>}}
%
% Commands for multiple indexes around a central token #1
% The names derive from "front up-down, back up-down" of #1 (it better be read as "left up-down, right up-down") indicating 
% the order in which indexes are passed starting with #2 (left-up or front-up). The only cool stuff about these commands is 
% that it reduces the space between up-down left indexes and the following token.
\newcommand{\fudbud}[5]{{\!\;}^{#2}_{#3}\!\!#1^{#4}_{#5}}
\newcommand{\fubu}[3]{{\!\;}^{#2}\!\!#1^{#3}}
\newcommand{\fdbd}[3]{{\!\;}_{#2}\!\!#1_{#3}}
\newcommand{\fdbu}[3]{{\!\;}_{#2}\!#1^{#3}}
\newcommand{\fubd}[3]{{\!\;}^{#2}\!#1_{#3}}
%
% put a small hat on operators!
\providecommand{\hatop}[1]{\ensuremath{\hat{\mathop{\operator@font #1}\nolimits}}}
%
% A small macro for generating uppercased letters of specific math font (mathfrak).
\let\op@format\mathfrak
% \let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%
% Jacobi elliptic functions as operators
\DeclareMathOperator{\jsn}{sn} % to replace duplicates above!
\DeclareMathOperator{\jcn}{cn}
\DeclareMathOperator{\jdn}{dn}
\DeclareMathOperator{\jns}{ns} % 1/sn(u)
\DeclareMathOperator{\jnc}{nc} % 1/cn(u)
\DeclareMathOperator{\jnd}{nd} % 1/dn(u)
\DeclareMathOperator{\jsc}{sc} % sn(u)/cn(u)
\DeclareMathOperator{\jsd}{sd} % sn(u)/dn(u)
\DeclareMathOperator{\jdc}{dc} % dn(u)/cn(u)
\DeclareMathOperator{\jds}{ds} % dn(u)/sn(u)
\DeclareMathOperator{\jcs}{cs} % cn(u)/sn(u) 
\DeclareMathOperator{\jcd}{cd} % cn(u)/dn(u)

% Pre-formatted special text chunks
\providecommand{\ie}{\textit{i.e.}}
\providecommand{\eg}{\textit{e.g.}}
\providecommand{\etal}{\textit{et al.}}



